MIGHTEE-HI: Discovery of an HI-rich galaxy group at z = 0.044 with MeerKAT

We present the serendipitous discovery of a galaxy group in the XMM-LSS field with MIGHTEE Early Science observations. Twenty galaxies are detected in HI in this $z\sim0.044$ group, with a $3\sigma$ column density sensitivity of $N_\mathrm{HI} = 1.6\times10^{20}\,\mathrm{cm}^{-2}$. This group has not been previously identified, despite residing in a well-studied extragalactic legacy field. We present spatially-resolved HI total intensity and velocity maps for each of the objects, which reveal environmental influence through disturbed morphologies. The group has a dynamical mass of $\log_{10}(M_\mathrm{dyn}/\mathrm{M}_\odot) = 12.32$, and is unusually gas-rich, with an HI-to-stellar mass ratio of $\log_{10}(f_\mathrm{HI}^\mathrm{*}) = -0.2$, which is 0.7 dex greater than expected. The group's high HI content, spatial, velocity, and identified galaxy type distributions strongly suggest that it is in the early stages of its assembly. The discovery of this galaxy group is an example of the importance of mapping spatially-resolved HI in a wide range of environments, including galaxy groups. This scientific goal has been dramatically enhanced by the high sensitivity, large field-of-view, and wide instantaneous bandwidth of the MeerKAT telescope.

==> abstract.tex <==
Environment is a key driver of galaxy evolution, which is prominently seen in well-studied rich, massive clusters that reveal clear trends in galaxy morphology, star formation rate, and neutral gas content with cluster radius. However, galaxy groups, which occupy dark matter halos with virial masses of order $10^{12-14}$\,M$_\odot$, are an important, yet more difficult to identify class in the continuum between individual field galaxies and the richest clusters. Observations of neutral hydrogen emission offer a unique approach to both their identification, as well as a means to a more holistic investigation, of morphology and group formation. The study of spatially-resolved \hi\ in a wide range of environments, including galaxy groups, will be dramatically enhanced by the high sensitivity, large field-of-view, and wide instantaneous bandwidth of the newly commissioned MeerKAT telescope. The MIGHTEE survey of several extragalactic legacy fields is particularly adept at this, enabling \hi morphological and dynamical measurements over a large cosmological volume. We present an early example of this, the serendipitous discovery of a galaxy group in the XMM-LSS field with MIGHTEE Early Science observations. %This survey is one of the first deep, large-area, blind, interferometric surveys for \hi ever undertaken, extending our knowledge of the \hi universe to $z = 0.6$. 
Twenty galaxies are detected in \hi in this $z\sim0.044$ group, with a $3\sigma$ column density sensitivity of $N_\mathrm{HI} = 1.6\times10^{20}\,\mathrm{cm}^{-2}$. We present \hi total intensity, velocity maps, and spectra for each of the objects, that reveal environmental impact through disturbed morphologies that are spatially resolved with MeerKAT. This early example is likely one of many as the full MeerKAT MIGHTEE survey progresses. This will enable the study of \hi\ in a wide range of environments and increase our understanding of its role in galaxy evolution. %of many to come as the MIGHTEE survey continues its observations of several extragalactic fields at significantly finer velocity resolution ($\sim5$\kms) than was available to these early science data ($\sim44$\kms), increasing the total number of known \hi galaxy groups and the scientific yield from each. 

We present the serendipitous discovery of a galaxy group in the XMM-LSS field with MIGHTEE Early Science observations. Twenty galaxies are detected in \hi in this $z\sim0.044$ group, with a $3\sigma$ column density sensitivity of $N_\mathrm{HI} = 1.6\times10^{20}\,\mathrm{cm}^{-2}$. This group has not been previously detected, despite residing in the well-studied XMM-LSS field, and is an early example of how the detection of spatially-resolved \hi in a wide range of environments, including galaxy groups, will be dramatically enhanced by the high sensitivity, large field-of-view, and wide instantaneous bandwidth of the newly commissioned MeerKAT telescope. We present \hi total intensity, velocity maps, and spectra for each of the objects, that reveal environmental impact through disturbed morphologies that are spatially resolved with MeerKAT. This group is unusually gas rich, with $\log(f_\mathrm{HI}^\mathrm{*}) = -0.2$, which is 1.1 dex greater than expected, suggesting that it is in the early stages of assembly. The discovery of this group is likely one of many, as the full MeerKAT MIGHTEE survey progresses. This will enable the study of \hi in a wide range of environments and increase our understanding of its role in galaxy evolution.
